HyperQuery: Beyond Binary Link Prediction

Groups with complex set intersection relations are a natural way to model a wide array of data, from the formation of social groups to the complex protein interactions which form the basis of biological life. One approach to representing such higher order relationships is as a hypergraph. However, efforts to apply machine learning techniques to hypergraph structured datasets have been limited thus far. In this paper, we address the problem of link prediction in knowledge hypergraphs as well as simple hypergraphs and develop a novel, simple, and effective optimization architecture that addresses both tasks. Additionally, we introduce a novel feature extraction technique using node level clustering and we show how integrating data from node-level labels can improve system performance. Our self-supervised approach achieves significant improvement over state of the art baselines on several hyperedge prediction and knowledge hypergraph completion benchmarks.

==> extra.tex <==
\section{Additional Information for Hyperedge Prediction}
Table~\ref{tb:std_pred} shows the mean test auc and standard deviation over 10 different train-test splits. We compare \textit{HyperQuery} with two other state of the art baseline methods. We find that our approach outperforms the other methods by a large margin, with high confidence.


\textbf{HyperQuery-minmax:} The best performing hyperedge prediction formulation presented in this paper. We use operator \textit{minmax} for the $\Omega$ aggregation function. We use 16 communities for our community detection step.

\textbf{NHP-minmax:} GCN based hyperedge prediction that can be used for directed and undirected hypergraphs. We used the minmax operator for this approach as well. 

\textbf{HyperSAGNN:} A self attention approach for hyperedge prediction that can only be used for undirected hypergraphs. We used random-walk basd approach.

 Comparing the performance of \textit{HyperQuery} with the baselines clearly demonstrates the effectiveness of leveraging community detection algorithms to improve prediction accuracy.  Our explanation for this is that community detection algorithms minimize global objectives, such as approximations of the NP-Hard multiway cut problem, whereas existing algorithms rely on purely local approaches like random walks and graph convolutions to learn salient features.  Our results demonstrate that partitioning with community detection can be an extremely powerful tool when one sets out to learn useful representations of hypergraph structured data.  

% 
\begin{table*}[htbp]
\caption{Area Under Curve (AUC) scores for hyperedge prediction.}
\label{tb:std_pred}
%\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{} & {\textbf{iAF1260b}}   &
 {\textbf{iJO1366}}&{\textbf{USPTO}} &{\textbf{DBLP}} \\ 
  &
  \multicolumn{1}{l}{AUC} &
 \multicolumn{1}{l}{AUC} &
  \multicolumn{1}{l}{AUC} &
  \multicolumn{1}{l}{AUC}  \\

  
\midrule
%Baseline & 62.4 $\pm .4$ & 60.4$\pm 1.$  & 65.5$\pm .1$   & 65.1$\pm 1.$  \\
HyperQuery-minmax & \textbf{72.2 $\pm .5$} & \textbf{68.5$\pm 1.$}  & \textbf{75.7$\pm .1$}   & \textbf{72.0$\pm 1.$}  \\
NHP-minmax & 64.3 $\pm 3.$   & 63.2 $\pm 2.$   &  74.2 $\pm 2.$  & 69.2  $\pm 2.$ \\
Hyper-SAGNN& 60.1 $\pm 1.$  & 56.3 $\pm 2.$ & 67.1 $\pm 1.$   & 65.2  $\pm 1.$ \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> txt/hyperedge_prediction.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[page=11,width=\textwidth]{fig/hyperquery_icml.pdf}
    \caption{ Generating Useful Labels using clustering: Not all hypergraph data comes with labels (\emph{left}). So far our approach has depended on having categorical labels on the edges and nodes.  We leverage hypergraph clustering to first assign cluster id as labels to the nodes, obtaining an initial cluster assignment $h^0_v$ (\emph{center}), which we then propagate to the hyperedges via Max Pooling (\emph{right}) in order to obtain the initial edge cluster assignment $h^0_e$.} % for pretext training.   }
    \label{fig:labeling_from_clusters}
\end{figure*}


\section{Hyperedge Prediction}
\label{sec:pred}
The second problem that we are addressing in this paper is the task of \textit{hyperedge prediction}, i.e. given an \emph{simple} hypergraph and set of nodes $(v_1,..,v_n)$,  predict whether this tuple forms a hyperedge. % The key difference between this problem and hyperedge classification is that in the latter problem, the hyperedge is known to exist. 

In this setting, there is no additional label data such as knowledge hypergraphs and thus inference must be computed entirely from the hypergraph structure.  Thus if we want to make use of a flow based approach, we need a way of computing a useful initialization.  Our insight is that useful initial categorical embeddings can be found by existing clustering algorithms.  

% The naive way of solving hyperedge prediction is to adapt the algorithm in Section~\ref{sec:classification}. Training is performed with actual hyperedges as well as with negative hyperedges ({\em i.e.}, node tuples that do not constitute hyperedges) that are assigned a label that is distinct from the labels in the dataset.
% We can then use the same algorithm (Equations \ref{eq:2},\ref{eq:3}) to solve hyperedge prediction. However, as we show in Section~\ref{sec:exp}, this approach does not perform well. The reason is that hyperedge prediction is a more complicated task than classification and requires more feature extraction and knowledge about the structure of our hypergraph. Specifically, in Section~\ref{sec:classification}, we are using hyperedge labels as our initial hyperedge features. However, the use of such features faces two challenges. First, the number of labels in hypergraph datasets is usually small. Second, even if we have many labels, these labels usually do not contain information about the link structure of the hypergraph. 

% To address these problems, we propose a labeling mechanism where the label of a hyperedge contains information regarding the structure of a hypergraph. Once we obtain these labels, we can use the message-passing scheme explained in Section~\ref{sec:classification} to optimize these initial features.





\subsection{Feature Extraction using Clustering}
\label{subsec:label}
One way to learn an embedding that captures meaningful structural information about a hypergraph is to run random-walk based algorithms such as node2vec~\cite{node2vec}. Previous works on hyperedge prediction such as HyperSAGNN~\cite{hypersagnn} and NHP~\cite{nhp} use node2vec to first learn feature vectors for nodes of a hypergraph represented in a variety of ways. Then, they improve these features using attention-based methods. However, such methods have a number of drawbacks:
\begin{enumerate}
    \item They do not learn the correlation between nodes that do not appear in the same random walk and may require many samples to capture evidence of weak correlations.
    \item Random walks explore only the local properties of the hypergraph, optimization might get stuck in local minima.  
    \item Random walks on hypergraphs mix very quickly due to high edge degree and thus even if an algorithm provably converges, computing this answer might not be practical in practice.
    \item There is no standard practice for how to transfer node level features into a feature vector per hyperedge, which we needed for the hypergraph convolution operator presented in section~\ref{subsec:full_op}.  
\end{enumerate}

It occurred to us that instead, it is possible to use state-of-the-art partitioning based clustering tools as an alternative approach for pre-computing features.  While clustering is a well studied problem in ML, for instance it has been used in link prediction as early as in 2015~\cite{link_prediction_community_detection}, it is not used by any of the state-of-the-art hyperedge prediction tools today, and we believe that this approach to generating intrinsically coherent features merits wider adoption, given the simplicity and effectiveness of the approach we evaluate in this paper.  

In particular, for our HyperQuery flow, we want to recover an initial label assignment that is ``smooth'' with respect to the underlying hypergraph topology.  To do this, we run a clustering  algorithm that partitions the nodes of the hypergraph into clusters. Each cluster of nodes is given a unique integer id.  To transfer these labels onto hyperedges, we perform a max-pooling step (described in more detail in Figure~\ref{fig:labeling_from_clusters}).  In particular, after performing clustering, we obtain a set of features $h_e^0$ and $h_v^0$ for every node and hyperedge in the input hypergraph.  These features are then used as initialization for the graph convolution operator we describe below.

% and if most of the nodes in hyperedge $h$ belong to community $c$, the initial label of $h$ can be set to the one-hot encoding of $c$. We call this the {\em community} of the hyperedge. In the actual implementation, we use an extension of this idea that is described later.



\textbf{Cut-Metric for Hypergraphs.} For our purpose, we can use any clustering algorithm. In our experiments, we use a multilevel clustering algorithm that partitions nodes into a given number of clusters while minimizing the hyperedge cut, defined below. While there is not a unique canonical way to define a hyper-edge cut, this approach worked well and exposes the number of clusters as a hyper-parameter to the system. 

\begin{align}
     cut(H,C) =  \sum_{e} (\lambda_e(H,C) - 1)\label{eq:6}
\end{align}

Here, $H$ is the hypergraph, $C$ is the partition of nodes into clusters, and $\lambda_e(H,C)$ is the number of clusters that hyperedge $e$ spans. Intuitively, nodes that belong to the same cluster are considered similar. This is similar to approaches like node2vec in which nodes that appear in the same random walk are considered to be similar. %Using clustering lets us exploit the global structure of the hypergraph, whereas random walk methods exploit only local information. 





\section{Optimizing The Hyperedge Convolution Operator}

Here we outline a few important technical details that significantly improve our framework.

\subsection{Node Cluster as a Feature}

%Below, we relate the information we gain via community detection to random walks in a connected hypergraph:
%\begin{claim}
%If node \textit{a} and \textit{b} are in the same community, there is a random walk from node \textit{a} to \textit{b} and vice versa that does not contain nodes in different communities. 
%The distance of this random walk is less than $|V| / P$ where $|V|$ is the number of nodes and $P$ is the number of partitions. The proof is in appendix. 
%\end{claim}


% In principle, we can just use the one hot vector of the cluster id of a hyperedge as its initial feature vector. However, this scheme does not capture correlations between different clusters. In particular, if a hyperedge has nodes in several clusters, only the cluster with the largest number of nodes of that hyperedge is represented in the one-hot vector. 

The initial aggregation step $AGG$ in our convolution operator comes from the idea that a reasonable first way to think about creating embeddings for hyperedges is to simply average node embeddings.  However, this simple measure fails to capture important information regarding the distribution of node embeddings within a hyperedge.  

To fix this problem, we augment every node feature vector with the a one-hot encoding of the node cluster id, as seen in Equation~\ref{eq:7}:
\begin{align}
h_{v}^k &= CONCAT\{ AGG\{{h_e^{k-1}, \forall e \in \mathcal{N}(v)}\}, x_v\} \label{eq:7}
\end{align}
where $AGG(.)$ is an aggregation function, and $x_v$ is the one-hot partition id of a node. If nodes of a hypergraph have features themselves, these features can also be concatenated with $x_v$. 


% \section{BLAH}
% Our final scheme for hyperedge message passing with both optimizations turned on is the following:
% \begin{align}
% h_{v}^k &= CONCAT\{ AGG\{{h_e^{k-1}, \forall e \in \mathcal{N}(v)}\}, x_v\} \label{eq:8}\\
% \Omega^k_e &= \Omega\{h_v^k ,\forall v \in \mathcal{N}(e)\} \label{eq:9}\\ 
% h_e^k &= \sigma(W^k \cdot  flat(\Omega^k_e \Omega^{k^T}_e)) \label{eq:10} 
% % h_e^k &= \sigma(W^k \cdot  concat(flat(\Omega^k \Omega^{k^T}),\Omega^k_{mean} )) \label{eq:temp}
% \end{align}


% where $\Omega$ is an aggregation function, $flat(.)$ flattens the correlation matrix and stores it in a column vector, $AGG(.)$ takes the element-wise mean of the hyperedge feature vector, $x_v$ is the feature vector of node $v$, and $W^k$ is the trainable weight matrix. The effect of different choices of summary functions $\Omega$ is experimentally evaluated in Section ~\ref{sec:exp}.

\subsection{Choosing the Right $\Omega$}
\label{subsec:omega}

% In figure~\ref{fig:zoo} we illustrate the zoo of statistical features that we evaluated.  In our paper we focused on evaluating each statistical feature separately in order to more clearly illustrate their relative effectiveness for our benchmark tasks.  In future work, it would be interesting to explore more complex and potentially learned approaches to this aggregation step as well.  An illustrated zoo of different choices of $\Omega$ that we tried can be found in Figure~\ref{fig:zoo}.

In this work, we evaluate three different types of summary statistics for $\Omega$.  A component-wise mean, a component-wise variance, and a sort of ``robust variance'' estimator we call \textit{minmax} (element-wise difference of maximum and the minimum values of the vectors) similar to the one used in NHP~\cite{nhp} to achieve state of the art performance.  Intuitively, when $\Omega$ is the mean, convolution maps hyperedges to the average embedding of constituent nodes, whereas the variance measures how correlated different nodes are with each other.  In our experiments in Section \ref{sec:exp}, we find that for the hyperedge prediction, \textit{minmax/variance} performed better as a choice of $\Omega$ whereas in knowledge hypergraph completion, \emph{mean} worked better.  


We also augment these aggregations to better capture the correlation between different labels/communities by introducing a bilinear aggregation layer~\cite{bilinear}. Bilinear aggregation has significantly improved visual concepts recognition~\cite{bilinear2}, and in practice also generally improves the accuracy of our results. Specifically, \textit{we create an auto-correlation matrix by multiplying a hyperedge feature vector by itself}. This matrix has dimension $d \times d$, which we then flatten. 

% \begin{figure*}[h]
% \centering
%     \includegraphics[page=16,width=.8\textwidth]{fig/hypergraph_embed_post_submission.pdf}
%     \caption{ Learning $W^1$.  Given a hypergraph with labels on nodes and edges, we experiment with a zoo of choices for $\Omega$.  In this illustration, we convolve once, multiply by $W^1$ and $\sigma$ and then pass through a fully connected layer to return to a space of the same dimension of hyperedge types.  Finally we then train as an autoencoder.}

%     \label{fig:zoo}
% \end{figure*}
% \subsection{Augmented Convolution Operator}
% \label{subsec:full_op}
% % $$ \ell^0$$ 
% $$\Omega^k_v  $$ $$  \Omega^k_e  $$
% $$\Omega^0_v  $$ $$  \Omega^0_e  $$

Our final scheme for hyperedge message passing is the following:
\begin{align}
%h_{v}^k &= CONCAT\{ AGG\{{h_e^{k-1}, \forall e \in \mathcal{N}(v)}\}, x_v\} \label{eq:8}\\
\Omega^k_e &= \Omega\{h_v^k ,\forall v \in \mathcal{N}(e)\} \label{eq:8}\\ 
h_e^k &= \sigma(W^k \cdot  flat(\Omega^k_e \Omega^{k^T}_e)) \label{eq:9} 
% h_e^k &= \sigma(W^k \cdot  concat(flat(\Omega^k \Omega^{k^T}),\Omega^k_{mean} )) \label{eq:temp}
\end{align}



Where $h_{v}^k$ is computed using Equation~\ref{eq:7}, $\Omega$ is an aggregation function, $flat(.)$ flattens the correlation matrix and stores it in a column vector, %$AGG(.)$ takes the element-wise mean of the hyperedge feature vector,$x_v$ is the feature vector of node $v$, 
and $W^k$ is the trainable weight matrix. The effect of using different aggregation functions $\Omega$ is explored empirically in Table~\ref{tb:prediction}.

% \subsection{Negative Sampling}
% \label{subsec:bilinear}

% Once trained, this scheme can be used as a pretext task to generate the representation of the hyperedges. We then apply a fully connected layer on them to generate logits to train cross entropy loss. We train the linear classifier using the frozen hyperedge representations. We use a similar approach to NHP~\cite{nhp} to generate negative samples, i.e for each hyperedge $e$, we create a negative hyperedge $\Tilde{e}$ by having half of nodes sampled from $e$ and the remaining from $V - e$. This sampling method is inspired by chemical reaction datasets. 


\textbf{Time complexity.} We analyze the time complexity of our framework (Equations \ref{eq:7}, \ref{eq:8},and \ref{eq:9}) in terms of the size of the hypergraph, assuming the number of relations (types) is independent of the size of the hypergraph. Let $m$ denote the number of hyperedges and $n$ denote the number of nodes. Let $deg (v_i)$ denote the degree of node $v_i$ and let $\Tilde{\Delta}$ denote $max_{1\leq i\leq n} deg (v_i)$. For Equation \ref{eq:7}, our framework takes  $O({n\cdot \Tilde{\Delta}})$ time.
For Equation~\ref{eq:8}, let $deg (e_i)$ denote the degree of hyperedge $e_i$ and let $\Delta$ denote $max_{1\leq i\leq m} deg (e_i)$.  Equation~\ref{eq:8} takes $O({m\cdot \Delta})$ time. Finally, the time complexity of Equation~\ref{eq:9} is constant since the number of labels is independent of the size of the graph. Overall, our framework takes $O({m\cdot \Delta}) + O({n\cdot \Tilde{\Delta}})$.





==> txt/knowledge_hgraph.tex <==
%\section{A Spectral Perspective}
\label{sec:analysis}

\section{Hyperedge Convolution Operator}
\label{sec:classification}
% We begin with the question of how one might build a system to ``answer'' hyper-queries. Given a collection of nodes, our HyperQuery oracle will answer questions such as whether these nodes are related. Ultimately, our goal is to 
% perform hyperedge prediction on a collection of nodes.

In this section, we start by studying the question of inference in knowledge hypergraphs, where a vector of data is stored on entities and relations. We present an approach for defining trainable convolutions on hyperedges which is well suited for performing inference for knowledge hypergraph completion. In the next section, we will discuss the pre-processing approach that completes our framework for performing hyperedge prediction on simple hypergraphs.






Our hyperedge convolution operator is motivated by the intuition of trying to learn an embedding for hyperedges given their labels.  In this setting, we might imagine using some statistical measure $\Omega$ (like mean or variance) to summarize the labels in the neighborhood of each hyperedge, and then training a MLP layer based on these summary statistics, as illustrated in equation~\ref{eq:1} and figure~\ref{fig:n2e}. 


% \begin{align}
% h_v^0 \\
% h_e^0
% \end{align}

\begin{align}
%m_{\mathcal{N}(e)}^k &= AGGREGATE({h_w^{k-1}, \forall w \in \mathcal{N}(e)}) \label{eq:1}\\
N2E(S,h_v^{k-1}) = h_S^k &= \sigma(W^k \cdot \Omega \{h_v^{k-1}\forall v \in S\}) \label{eq:1}
\end{align}

In particular, this equation defines a \emph{node2edge} convolution operator, as long as we take $S = \mathcal{N}(e)$ (neighborhood of hyperedge $e$) for a known hyperedge $e$.  That said, we can perform $N2E$ summarization on sets of of nodes which are not known to share a hyperedge.  In fact, this idea will enable our formulation to generalize to unknown data after appropriately training the weight matricies $W^k$ and nonlinear activations $\sigma$.





This approach to generating hyperedge embeddings is natural and simple, but the problem is that it depends on there existing high quality node level data $h_v$.   In this paper we are also interested in studying the problem of unlabeled hypergraphs, and accordingly are interested in performing several convolution steps in order to improve performance when initial node labels data is unreliable.  

To this end, we define an \emph{edge2node} convolution, which is formulated as a harmonic mean of neighboring edge embeddings using the function $AGG$.  
\begin{align}
%E2N(v_i, h_{e}^k) = h_{v_i}^k&= AGG({h_e^{k-1}, \forall e \in \mathcal{N}(v_i)}) \label{eq:2}
E2N(S, v_i) = h_{v_i}^k&= AGG({h_e^{k-1}, \forall e \in \mathcal{N}(v_i)}) \label{eq:2}
\end{align}
Where now $S$ is a set of hyperedges in the neighborhood of node $v_i$.
%Accordingly, our full \emph{edge2edge} convolution operator can be written as in equation~\ref{eq:3}.  
Now suppose that $h_v^k$ is the set of one hot vector of labels on all the nodes and $h_e^k$ on the edges after the $k^{th}$ step of convolution.  Then we can define a full \emph{edge2edge} convolution operator as follows:  

\begin{align}
E2E(e_i, h_e^{k-1}) &= N2E(\mathcal{N}(e_i), h_v^{k} )\\
 &=\sigma(W^k \cdot \Omega (\{h_v^k \forall v \in \mathcal{N}(e)\}) ) \label{eq:3}
\end{align}
 

% In words, for each node $v$ in hyperedge $e$, we aggregate along it's hyperedge neighbor features to calculate $h_v$. Then, for each hyperedge \textit{e}, we aggregate the messages from its nodes ({\em i.e.}, $h_v \forall v \in \mathcal{N}(e)$), using a \emph{summarization} function $\Omega(.)$ as shown above.  Finally, we have a hidden ``deconvolution'' layer and a non-linearity. 
% The $h_{v_i}^k$ in eq.~\ref{eq:2} amounts to a ``mean-field'' embedding of each node $v_i$ as the average of a sampling of the data stored on the hyperedges it is connected to.

% However, when representing hypergraphs as bipartite graphs, one is compelled to similarly define 


%Our approach here is to define a measure we call $hs^1_q$, the first \emph{Harmonic Statistic} of a query set $q$, to be a vector in $R^n$, computed accordingly: 
%\begin{align}
%m_{\mathcal{N}(e)}^k &= AGGREGATE({h_w^{k-1}, \forall w \in \mathcal{N}(e)}) \label{eq:1}\\
%h_{v_i}^1 = AGG\left(h_e \forall e \in \mathcal{N}(v_i) \right) \\
%hs^1_q = hs(q) = \Omega( h_{v_i}^1 \forall v_i \in q) \label{eq:1}
%\end{align}



% To fully unlock the power of modern machine learning, we set out to create a trainable system. In fact, we improve on Equation ~\ref{eq:1} and propose something more general.  A flexible, composable, trainable, hyperedge message-passing based (i.e. scalable) operation for learning to answer HyperQueries. 



% \begin{align}
% h_{v}^k &= AGG({h_e^{k-1}, \forall e \in \mathcal{N}(v)}) \label{eq:2}\\
% hs_e^k &= \Omega (\{h_v^k \forall v \in \mathcal{N}(e)\}) \label{eq:3}\\
% h_e^k &= \sigma(W^k \cdot hs_e^k ) \label{eq:4}
% \end{align}


% for each node associated to a , we first \emph{aggregate} the representations of all of the edges within its ``receptive field'' by averaging.  Intuitively, this message passing based aggregation step can be thought of a \emph{diffusion process} or a \emph{flow}, which averages and symmetrizes the edge level data by effectively performing a step of Laplacian smoothing.  In the second part we \emph{summarize} the distribution of aggregated node labels with a function $\Omega$.


% To this end, we define 


% As hyperqueries must be defined as hyperedges, our system must store data on hyperedges.  The more well studied Node-based GCN frameworks cannot be used directly for our problem since the entities of interest to us are the hyperedges and not the nodes of the hypergraph. A naive solution is to convert the hypergraph to the dual clique graph in which the nodes of the new graph represent the hyperedges of the original graph, and nodes representing two hyperedges are connected by an edge if the corresponding hyperedges have at least one node in common in the original hypergraph. We can then apply traditional message passing algorithm on this new graph using the following update rule:  
% \begin{align}
% %m_{\mathcal{N}(e)}^k &= AGGREGATE({h_w^{k-1}, \forall w \in \mathcal{N}(e)}) \label{eq:1}\\
% h_e^k &= \sigma(W^k \cdot \Omega \{h_v^{k-1}\forall v \in \mathcal{N}(e)\}) \label{eq:1}
% \end{align}

% \begin{figure}
%     \centering
%     \includegraphics[page=9,width=\textwidth]{hypergraph_embed.pdf}
%     \caption{We use message passing to aggregate distributional features on each hyperedge.  We start by assuming that we have categorical labels on nodes and hyperedges $\ell^0$, or computing them using the process described in figure~\ref{fig:labeling_from_communities}, (\emph{left}).  Next we observe that by first passing edge labels onto vertices we will accumulate salient local features about label distributions (\emph{center}).   Performing a second message passing and aggregation step (\emph{right}) can be interpreted as assigning to each hyperedge an aggregate measure of the labels assigned to both the nearby nodes and edges.   }
%     \label{fig:init_edge_embedding}
% \end{figure}
%, notated as the neighborhood $\mathcal{N}(v_i)$. Correspondingly, we take $AGG$ to be a component-wise mean operator.  $\Omega$ is taken as differentiable \emph{summarization} function, we test several choices of this measure in our work.



%\subsection{From Harmonic HyperQuery Statistics to Learned Convolutions}

%Second, to fully unlock the power of modern machine learning, we set out to create a trainable system.  To this end, we present an operator which can be directly used to attempt to invert from $hs_q^1$ in ~\ref{eq:1} to its training label in a supervised learning setting. % In this setting we are actually directly learning a \emph{deconvolution}, but in practice we prefer to iterate this process in order to obtain a ``deeper'' model which performs an iterative smoothing/sharpening process.  



% , $\sigma$ is the non linearity function, and $W^k$ is a learned weight matrix. Intuitively, we first aggregate the messages that come from neighboring hyperedges and then update the embedding of hyperedge \textit{e}. However, this approach is lossy because the nodes of the hypergraph are not considered in the embedding, and this does not let us differentiate between hyperedges that have many nodes in common from hyperedges that have very few nodes in common. 
%This is important since the message that comes from a hyperedge that has many node in common with hyperedge \textit{e} should be different that the hyperedge that has only one node in common with hyperedge \textit{e}.



%The above scheme relies on node-based message passing. However, we are interested in message passing between hyperedges in order to be able to do prediction over hyperedges. 
%The way we fix this problem in our scheme is to define a node's message based on its hyperedges i.e. the aggregation of feature embedding of the hyperedges it belongs to. 

%When we have reliable edge labels,
In a knowledge hypergraph, we can effectively learn the hidden weights $W^k$ by choosing the initial feature $h^0_e$ of a hyperedge $h_e$ to be the one hot vector of its type, and building up an autoencoder style problem.  % Equation~\ref{eq:2} uses these values to compute initial embeddings for nodes. These values are updated iteratively for some number of rounds using Equations~\ref{eq:3} and \ref{eq:4}.   
By repeating this iteration twice, we already arrive at an effective tool for knowledge hypergraph completion which generalizes to unseen data far better than benchmark approaches.  In the experiments, we outline our performance relative to other benchmarks.  We achieve this performance with a straightforward model where we simply treat the output $h_e^2$ as a predicted class label $\mathcal{P}(e)$.  From there we minimize the loss below as a function of hidden layer weights $W^1$ and $W^2$.  
\begin{align}
 \mathcal{L} = \sum_{e \in \mathcal{D}} \mathcal{J}( \mathcal{P}(e), \mathcal{G}(e)) \label{eq:5}
\end{align}

In our objective function, we take $\mathcal{J}(.)$ to be the cross entropy loss, $e$ to be a hyperedge in the training dataset $\mathcal{D}$, $\mathcal{P}(e)$ is the predicted type of hyperedge $e$, and $\mathcal{G}(e)$ is the actual ground truth type (relation) of hyperedge $e$ in the dataset. % This training process is illustrated in figure~\ref{fig:pipeline}.


This concludes the first part of our approach to learning useful representations of Hyper-queries.  Intuitively, one can think of our $E2E$ operator as first performing a step of diffusion where labels get averaged with their neighbors, followed by a ``deconvolution'' step using learned weights.  This algorithm is straightforward to implement and effective at capturing high-order structures present in data. 

% One way to think about this is that the MLP is tasked with inverting the diffusion process onto a target space of types.  

%  that by simply minimizing a cross entropy loss $\mathcal{L}$ between ground truth labels $\mathcal{G}(e)$ from the training set, and twice-convolved hyperedge vectors $h_e^2$, and backpropogating through the hidden layers:   

% \begin{figure}[h]
% \captionsetup{font=normalsize,labelfont={bf,sf}}
% \captionsetup[sub]{font=footnotesize,labelfont={bf,sf}}

% \centering

% \begin{subfigure}{0.3\textwidth}
%   \caption{The \emph{community} of a hyperedge $e$ is the set of neighboring nodes $\mathcal{N}(e)$}
%      \includesvg[width=\columnwidth]{fig/sep_log_community}
%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community_flow}
%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community_agg}
%     \label{subfig:community}
% \end{subfigure} 
% \hfill
% \begin{subfigure}{0.3\textwidth}
%   \caption{ $AGG$ can be considered as a smoothing operator, averaging the embedding $h^k_e$, of each edge $e$ in $\mathcal{N}(v)$.}
    
%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community}
%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community_flow}
%      \includesvg[width=\columnwidth]{fig/sep_log_community_agg}
%     \label{fig:agg}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\textwidth}
%     \caption{$\Omega$ aggregates node level data which gets transformed into an edge representation. }% We discuss different choices of $\Omega$ later in the paper.}

%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community}
%      \includesvg[width=\columnwidth]{fig/sep_log_community_flow}
%     %  \includesvg[width=0.31\columnwidth]{fig/sep_log_community_agg}

%     \label{subfig:flow}
% \end{subfigure}

%     \caption{  Something something }
%     \label{fig:conv_ops}
% \end{figure}





